Vision Transformers for Weakly-Supervised Microorganism Enumeration

Microorganism enumeration is an essential task in many applications, such as assessing contamination levels or ensuring health standards when evaluating surface cleanliness. However, it's traditionally performed by human-supervised methods that often require manual counting, making it tedious and time-consuming. Previous research suggests automating this task using computer vision and machine learning methods, primarily through instance segmentation or density estimation techniques. This study conducts a comparative analysis of vision transformers (ViTs) for weakly-supervised counting in microorganism enumeration, contrasting them with traditional architectures such as ResNet and investigating ViT-based models such as TransCrowd. We trained different versions of ViTs as the architectural backbone for feature extraction using four microbiology datasets to determine potential new approaches for total microorganism enumeration in images. Results indicate that while ResNets perform better overall, ViTs performance demonstrates competent results across all datasets, opening up promising lines of research in microorganism enumeration. This comparative study contributes to the field of microbial image analysis by presenting innovative approaches to the recurring challenge of microorganism enumeration and by highlighting the capabilities of ViTs in the task of regression counting.

==> tables/MAE_reduced.tex <==
\begin{table*}
\centering
\caption{Average mean absolute error, root mean square error, and floating point operations per second. The best result is shown in bold and the second best in underlined. Separated are the three types of architectures chosen in the experiments: traditional methods, state-of-the-art, and ViT backbone implementations.}
\label{tab:models_performance}
\begin{tabularx}{0.6\textwidth}{
  >{\hsize=1.3\hsize\raggedright\arraybackslash}X
  *{8}{>{\hsize=0.94\hsize\centering\arraybackslash}X}
  >{\hsize=1.2\hsize\centering\arraybackslash}X} %{>{\hsize=1.5\hsize\raggedright\arraybackslash}X*{8}{>{\hsize=0.95\hsize\centering\arraybackslash}X}}%{>{\raggedright\arraybackslash}X*{9}{>{\centering\arraybackslash}X}} %{lccccccccc}
Architectures
& \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Fluorescent\\ Neuronal Cells\end{tabular}} & \multicolumn{1}{c}{VGG-Cells} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Human\\ Cancer Cells\end{tabular}}  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Fluorescent\\ Artificial Bacteria\end{tabular}}\\
\midrule
CNN Base       & 2.123                    & 6.212                  & 59.584                   & 43.282                    \\
CNN Medium     & 1.828                    & 4.991                  & 40.130                & 34.307                    \\
CNN Deep       & 1.566           & 1.827               & 52.507                & 24.987                   \\
ResNet50       & 1.508                    & \textbf{1.225} & \textbf{27.206} & \underline{22.030}  \\
ResNet101      & \textbf{1.400}  & \underline{1.311}  & \underline{30.497}  & 23.313               \\
\midrule
TransCrowd-G   & 2.011                    & 9.321            & 47.627       & 31.997              \\
TransCrowd-T   & 1.497                    & 2.585          & 58.152             & 22.563               \\
\midrule
CrossViT       & 1.634                   & 3.012            & 43.356              & \textbf{20.011}  \\
DeepViT        & \underline{1.464}           & 37.713         & 71.171             & 106.402                  \\
XCiT           & 1.654                    & 3.139          & 49.163                  & 27.158               \\
Parallel ViT   & 1.519                    & 2.400                & 44.972        & 23.736                \\
Vanilla ViT    & 1.541                    & 1.886            & 57.886              & 26.055            \\
\bottomrule

\end{tabularx}

\end{table*}


==> tables/datasets_table_reduced.tex <==
\begin{table*}[t]
\centering
\caption{Characteristics of the datasets used. The number of images refers to the size of the training and validation sets, the resolution refers to their original datasets, the ground truth is how they were originally labeled, and the count statistics show the total number of instances in all images of the dataset, and the minimum, average, and maximum number of instances per image.}
\label{tab:datasets_comparison}
\small
\renewcommand{\arraystretch}{1.0}
\begin{tabular*}{0.6\textwidth}{@{\extracolsep{\fill}}lccccc@{}}
\toprule
& &
\multicolumn{4}{c}{Count statistics} \\
\cmidrule(lr){3-6}
Dataset & 
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Number of\\ images\end{tabular}} & 


\text{Total number} & 
\text{Min} & 
\text{Ave} & 
\text{Max} \\ 
\midrule
Fluorescent Neuronal Cells      & $10000$    & $18475$       & $0$ & $2$     & $17$ \\
    VGG-Cells                   & $19294$      & $2480424$ & $1$ & $128$   & $317$ \\
Human Cancer Cells              & $1463$    & $201058$      & $0$ & $138$   & $410$ \\
Artificial Fluorescent Bacteria & $12000$    & $10963874$    & $0$ & $913$   & $1855$ \\ 
\bottomrule
\end{tabular*}
\end{table*}
